TestSpark: IntelliJ IDEA's Ultimate Test Generation Companion

Writing software tests is laborious and time-consuming. To address this, prior studies introduced various automated test-generation techniques. A well-explored research direction in this field is unit test generation, wherein artificial intelligence (AI) techniques create tests for a method/class under test. While many of these techniques have primarily found applications in a research context, existing tools (e.g., EvoSuite, Randoop, and AthenaTest) are not user-friendly and are tailored to a single technique. This paper introduces TestSpark, a plugin for IntelliJ IDEA that enables users to generate unit tests with only a few clicks directly within their Integrated Development Environment (IDE). Furthermore, TestSpark also allows users to easily modify and run each generated test and integrate them into the project workflow. TestSpark leverages the advances of search-based test generation tools, and it introduces a technique to generate unit tests using Large Language Models (LLMs) by creating a feedback cycle between the IDE and the LLM. Since TestSpark is an open-source (https://github.com/JetBrains-Research/TestSpark), extendable, and well-documented tool, it is possible to add new test generation methods into the plugin with the minimum effort. This paper also explains our future studies related to TestSpark and our preliminary results. Demo video: https://youtu.be/0F4PrxWfiXo

==> sections/4-future.tex <==
\section{Future steps}
Firstly, we aim to expand \tool's language support. Given the flexibility of the proposed approach for LLM-based test generation and the power of \idea, we can achieve this by implementing new test parsers and runners for each language.

Moreover, we want to assess the usability of our plugin and the usefulness of tests generated by each technique. We seek to gain insights into both the strengths and areas for improvement in the generated tests, as well as the \tool's features.  
Hence,  we are working to (i) enhance telemetry in \tool to collect feature usage statistics, and (ii) design and perform a UX study to answer the following research questions: \textbf{RQ1:} How useful the generated tests are for developers in their day-to-day testing practices? and \textbf{RQ2:} How is the usability of the \tool plugin?

In parallel, we keep improving the features in \tool (\eg allowing users to select more testing goals, such as integration between classes~\cite{derakhshanfar2022basic}).
In addition, we aim to combine different test generation methods to generate better unit tests in \tool (\eg combining SBT and LLM-based test generation).

